Dandelion: multiplexing Byzantine agreements to unlock blockchain performance

Permissionless blockchain protocols are known to consume an outrageous amount of computing power and suffer from a trade-off between latency and confidence in transaction confirmation. The recently proposed Algorand blockchain protocol employs Byzantine agreements and has shown transaction confirmation latency on the order of seconds. Its strong resilience to Denial-of-Service and Sybil attacks and its low computing power footprint make it a strong candidate for the venue of decentralized economies and business ecosystems across industries. Nevertheless, Algorand's throughput is still far from the requirements of such applications. In this paper, we empower Algorand's protocol by multiplexing its byzantine agreements in order to improve performance. Experiments on wide area networks with up to ten thousand nodes show a 4-fold throughput increase compared to the original Algorand protocol.

==> sections/approach.tex <==
Model And Goal
The system consists of a set of N nodes connected by a reliable peer to peer network. Each node communicates with its peers. In the network, the upper bound of message propagation delay is known, and it is Delta.

Nodes have access to standard cryptographic primitives to generate key pairs, produce message digest, and sign messages. Each node in the system knows the public key of all other nodes. Any message contains a signature and identity of the sender so that nodes can validate the messages.

In the system, we have correct and faulty nodes. Correct nodes always follow the protocol. Faulty nodes may violate the protocol in any possible way. In our system, the proportion of faulty nodes is less than or equal to 1/5N. All faulty nodes controlled by an adversary. 

Goal
We have the following goals which are the same goals with Algorand's consensus protocol.


Safety goal: With overwhelming probability, all users agree on the same transactions. More precisely, if one honest user accepts transaction A (i.e., it appears in the log), then
any future transactions accepted by other honest users will appear in a log that already contains A. This holds even for isolated users that are disconnected from the network.

Liveness goal: In addition to safety, Dandelion also makes progress (i.e., allows new transactions to be added to the log) under additional assumptions about network reachability.

Algorand and its blockchain protocol
Algorand is a Proof of Stake(PoS) public blockchain consensus algorithm. It is using Verifiable Random Functions(VRF), and a cryptographic sortition algorithm to elect leaders and committee members from consensus participants in a verifiably random manner. Any node with a stake in the system can participate in consensus. In each round, participants run a special consensus algorithm, Binary Agreement Start (BA*), to agree on blocks.

In Algorand, time is divided into successive epochs and in each epoch, there are elected leaders. An epoch consists of several steps (up to 255), and each step has committee members.  Users with stakes may be elected as leaders or committee members. A user may be elected to participate in consensus as a leader or committee member. A user may be elected more than once in a round for different roles (as a leader or as a committee member for any step)

Elections in Algorand are done locally by nodes using a VRF and cryptographic sortition. VRF is used to produce a random number in a verifiable manner using the seed and the secret key of the node. The source of the randomness is called as seed and each block in algorand has a seed field which is calculated with another deterministic function. The seed field of a block appended to blockchain is used as a randomness source for the elections of the next round. The output of the VRF is used to run the cryptographic sortition with the number of owned tokens of a user. The use of owned tokens (stake) protects the system against Sybil attacks because an attacker should have a huge amount of stake in the system to hijack the consensus which is very costly.  The result of the election can be verified by any node because all data is publicly available to verify the result of the election.

At the beginning of each round, any node runs the election algorithm to learn whether or not elected as leaders. Algorand selects more than one leader for each round (up to 70). The number of leaders is controlled by a protocol parameter which is threshold proposer. Any elected leader submits a block with proof of the election. Each block assigned a priority using a deterministic function. Nodes forward-only block with valid proofs and highest priority.  

A leader submits a second message which contains the hash of the block with the proof of election. This message is very small and propagates fast in the network. In each round using the small message nodes learn about available blocks in a short amount of time so that they can limit unnecessary block propagation.

After the leader election, each node waits for a short amount of time, which is another protocol parameter, to receive enough proposition to start the BA*. Each node starts BA* with the highest priority proposition it received. If a node does not receive the block with the highest priority in a predefined time interval, it starts the BA* with an empty block. BA* consists of two phases. In the first phase, nodes run a reduction algorithm to decrease the possible blocks from many to two(the empty block and a block with the highest priority). In the second phase, nodes run the Binary BA algorithm to agree on one of the two blocks which is produced by reduction. 

In each step of the algorithm,  any participant runs the election algorithm to learn whether it is elected as a committee member or not. An elected committee member votes in that step for a specific value, and the votes contain the proof of election. If the network synchronous, BA* produces a final result in 4 steps. If the network asynchronous BA* takes more than 4 steps (up to 255), and it produces a tentative result. A final result is final and it can not change. On the other hand, a tentative result may change in the future.

In Algorand, any elected node (a committee member or leader) sends a single message with the proof of election. The election result can be verified but it can not be produced by any other node because it requires secret information(secret key of the user). This construction protects nodes from denial of service attacks because the identity of an elected node(a committee member or leader) can not be known in advance.


We are ready to describe Dandelion.


==> sections/eval.tex <==
\section{Evaluation}\label{sec:evaluation}

We evaluate the Dandelion to answer the following questions quantitatively:

\begin{itemize}
    \item What is the optimum $\tau_{PROPOSER}$ value for Dandelion?
    \item How does round latency improved compared to Algorand?
    \item How much throughput gain does Dandelion provide on top of Algorand?
    \item How does Dandelion behave with different CC and macroblock sizes?
    \item Does  Dandelion scale?
    \item How does  Dandelion scale compared to Algorand?
    \item How Dandelion behaves with increased CC values?
\end{itemize}

%To answer these questions, we deployed our prototypes on Grid'5000, a large-scale and flexible testbed for experiment-driven research in all areas of computer science, with a focus on parallel and distributed computing. For each set of experiments, we booked a specific number of machines in the \textit{gros cluster} composed of 124 machines located in Nancy. Each machine comprises an Intel Xeon Gold 5220 18-core CPU, 96GiB of memory, and 25 Gbps intra network connectivity. 
%To emulate wide-area-network conditions, we cap the bandwidth of each Dandelion process to 20Mps using cgroups and traffic control rules, and we added 50 ms latency for each outgoing (round trip 100ms) packet using traffic control rules. 
%As in Algorand, we assigned an equal share of tokens to each node during experiments that maximizes the number of messages during each round. In all provided graphs, we plot the first quantile, median, and third quantiles. 

\subsection{Optimum Threshold Proposer Value for Dandelion }
In Algorithm, $\tau_{PROPOSER}$ value set to 26. This guarantees that there will be at least one and at most 70 leaders with a high probability\cite{AlgorandGoalgorand2021}.  In Dandelion, we are assigning a microblock index hence a batch of transactions to each elected leader.  Microblock index assignment is deterministic, and it relays on the  output of the leader election algorithm of Algorand which is not a deterministic algorithm.  We have conducted a set of experiments to find the minimum $\tau_{PROPOSER}$  value to assign each microblock index at least one leader. 

To find the minimum $\tau_{PROPOSER}$  value,  we have conducted a set of experiments on 10 machines with 100 nodes per machine (total 1000 nodes).  We deployed Dandelion with CC 20 and macroblock size 20MB.  
We vary  $\tau_{PROPOSER}$ values  from 10 to 100, and we have measured the size of appended macroblocks to the blockchain.

\begin{figure}
        \includegraphics[width=\columnwidth]{results/threshold_proposer_value.png}
        \caption{Round Latency}
        \label{fig:threshold_proposer_value}
\end{figure}

In the figure \ref{fig:threshold_proposer_value},  we have the $\tau_{PROPOSER}$ value on the X-axis,  and we have the average size of appended macroblocks on the Y-axis.  When we increase the $\tau_{PROPOSER}$ value from 10 to 90 average macroblock size increasing also. After $\tau_{PROPOSER}$ value 90, we are reaching the maximum macroblock size.

In the light of these experiments, we set $\tau_{PROPOSER}$ value to 100 in Dandelion implementation to utilize the capacity of macroblocks fully.

\subsection{Latency and Throughput}

In this section, we investigate the performance of \protoname in terms of latency for confirming a block, and effective throughput. We compare effective throughput and block confirmation latency figures of Dandelion with Algorand.

In our evaluation,  each round starts with leader election, and ends with appending a block to the blockchain.  The time between these two events is the latency we consider.  The throughput depends on the size of appended blocks, and block confirmation latency.  

In this set of experiments, we have used 10 machines from Grid'5000 with previouslşy provided specs, and we have deploy 100 Dandelion or Algorand node per machine which means 1000 nodes per deployed experiment. 

We have used different macroblock sizes from 1 MB to 24MB. We have change CC values from 1 to 20 for each macroblock size. During an experiment, macroblock size and CC values are kept constant. In plots CC1 values corresponds to classical Algorand values. CC values 2 and higher corresponds to Dandelion values.  In each experiment, we have run the experiment long enough to warm up  the system, and afterward, we collected data on each node. 

The figure \ref{fig:param_lat} shows the round latency for different macroblock sizes and CC values. When we increase the macroblock size from 1MB to 24MB round latency is increasing because in Algorand, and Dandelion nodes are waiting to receive the highest priority block before starting BA$\star$, and in the case of big blocks, receiving the block with the highest priority takes a longer time. In the case of Algorand, as we see in the figure \ref{fig:param_lat} with CC1,  the  round latency is increasing linearly with increased block size which means that using bigger blocks with Algorand causes an increase in confirmation latency.

In the figure \ref{fig:param_lat},  the latency values of Dandelion increases linearly with increased macroblock size on any CC value.  The increase is inversely proportional to CC values, and this alleviates the effect of round latency because the increase is not as dramatic as in Algorand. To append a 20MB block of transactions,  Algorand needs 110 seconds on the other hand Dandelion with CC 20 needs 32 seconds.



Figure \ref{fig:param_thr} shows how throughput changes by varying macroblock size and CC. When we increase the macroblock size it is expected to see higher throughputs but it is not the case because larger blocks takes longer to disseminate, and this limits throughput gain. We can observe this phenomenon easily in Algorand throughput measurements. Throughput values of Algorand does not increases with increased block size.

For Dandelion,  up to 4MB macroblock size,  all throughput values for different CC values are very close because dissemination of small microblocks take a longer time because of added latency to the channels to emulate WAN conditions.  When we increase  CC with macroblock size 4 we can easily observe the throughput gain. We obtain the best throughput value with 24MB macroblocks, and CC 20. In all plots CC16, and CC20 values are very close because the size of microblocks are very close to each other.


\subsection{Scalability experiments}

To determine how does \protoname scales in terms of throughput and latency when increasing the number of nodes in the system, we run another set of experiments where we vary the total number of machines involved from 10 to 100, deploying 100 Dandelion nodes per machines. In this experiment set, we used macroblocks with 20MB, and we set CC to 20.  We started with 1000 nodes, and we have added 1000 nodes (10 machines) in each iteration.

As we see in the figure \ref{res:scale_lat}, the latency of Dandelion is increasing with the increased number of nodes in the system. This is expected because with the increased number of nodes, the number of votes needed to have consensus on a block increasing. Also, with a bigger network, the time needed to disseminate a block is increasing so the round latency of Dandelion increasing.


When we increase the number of nodes in the system, we have observed a decrease in the throughput as in show in the figure \ref{res:scale_thr}. This was expected because of the increase in round latency.

Although, there is a drop in the throughput, and an increase in the latency with the increased number of nodes, this drop is small, and the system size is fairly big. We can conclude from this experiment set that deploying Dandelion with 10,000 nodes provides reasonable throughput that is 400Kb/s, and reasonable round latency that is less than 53 seconds.


% \begin{figure}
%     %\begin{subfigure}{\columnwidth}
%         \includegraphics[width=\columnwidth]{results/scale_lat.png}
%         \caption{Round duration}
%         \label{res:scale_lat}
%     % \end{subfigure}
%     % \newline
%     % \begin{subfigure}{\columnwidth}
%         \includegraphics[width=\columnwidth]{results/scale_thr.png}
%         \caption{Effective throughput}
%         \label{res:scale_thr}
%     % \end{subfigure}
%     % \caption{\protoname scalability}
%     %\label{res:scale}
% \end{figure}


\subsection{Reaching the limits of Dandelion}

\begin{figure}
        \includegraphics[width=\columnwidth]{results/limits_of_dandelion.png}
        \caption{Median throughput figures with CC32,  with different $\tau_{PROPOSER}$ values }
        \label{fig:limits_of_dandelion}
\end{figure}

In Dandelion, the CC parameter is the most important parameter that controls the throughput and latency characteristics of the system. In previous experiments, we observed that with increased CC values it is possible to increase throughput with a little increase in latency. The last question we have answered is what is the best performance we can be achieved by increasing CC value. To answer this question, we have conducted a set of experiments,  with 1000 Dandelion nodes that are deployed on 10 machines. 


In this set of experiments, we used three different macroblock sizes and we set the CC value to 32.  We run the same experiments with different high $\tau_{PROPOSER}$ values to guaranty full macroblocks.   On the figure \ref{fig:limits_of_dandelion}, we have macroblock size on the X-axis, and we have median throughput values on the Y-axis.  When we set CC as 32,  we could not observe a dramatic increase in throughput compared the CC 16 values on the figure \ref{fig:param_thr}. 


% To that end, 

% In experiments we replaced vote and block validations with sleep times in order to increase the number of deployed nodes. 
% Sleep times are calculated per machine because validations take less time with a powerful machine.


% \subsection{Setup}

% We conducted two sets of experiments to evaluate the performance and scalability of the proposition.

% In our experiments, we set the total available token in the system to 1.000.000, and we distribute the tokens equally to all nodes in the system.


% We conducted experiments using similar parameters with Algorand. 
% The figure 1 shows the parameters of classical Algorand.
% In our implementation we did not implement Seed refresh interval. 
% We set the threshold proposer to 100 to have enough leaders to fill the macroblocks. 
% We set the lambda block and lambda step timeouts to 60 and 120 seconds respectively.  
% Except for these changes, we have used the same parameters with algorand.

% \subsection{Performance Evaluations}

% To evaluate the performance of our proposition we have conducted a set of experiments and we have measured throughput and consensus latency figures. 
% We have run the experiments on G5K machine. 
% We have used XX physical machines with an Y core CPU and Z megabytes of memory. 
%Machines are connected with ZZZGigabits links. 
% We have deployed P processes per machine. 
% To emulate the WAN conditions, we capped the band width of each process to 20 Mbps using cgroups and TC traffic control rules. 
% We added 100 ms communication latency (RTT) between any two processes using TC traffic control rules.
% To evaluate the performance of the system, we had conducted a set of experiments by changing Macroblock size and concurrency constant.
% All experiments used the same configuration. We collected consensus latency, and throughput statistics to evaluate the performance of the system with varying macroblock size and CC.

% \subsection{Scalability}

% In this set of experiments, we set the macro block size to SS and concurrency constant value to CC, and we change the number of nodes in the system.
% We have used XX machines with a Y core CPU and ZZ MBs of memory. 
% Machines are connected with ZZZGigabits links.
% We limit the bandwidth and we added latency as in the previous set of experiments. 
% We started the experiments with K machines and in each iteration we increased the number of machines K. 
% We measured the consensus latency in each experiment. 



% Figure 4 shows the parameters in our prototype of Algo- rand; we experimentally validate the timeout parameters in section 10. 
% h = 80\% means that an adversary would need to control 20\% of Algorand’s currency in order to create a fork.
% By analogy, in the US, the top 0.1\% of people own about 20\% of the wealth [41], so the richest 300,000 people would have to collude to create a fork.
% $\lambda_{priority}$ should be large enough to allow block proposers to gossip their priorities and proofs. Measurements of mes- sage propagation in Bitcoin’s network [18] suggest that gos- siping 1 KB to 90\% of the Bitcoin peer-to-peer network takes about 1 second. We conservatively set $\lambda_{priority}$ to 5 seconds.
% $\lambda_{block}$ ensures that Algorand can make progress even if the block proposer does not send the block. Our experiments (§10) show that about 10 seconds suffices to gossip a 1 MB block. 
% We conservatively set $\lambda_{block}$ to be a minute.
% $\lambda_{step}$ should be high enough to allow users to receive messages from committee members, but low enough to allow Algorand to make progress (move to the next step) if it does not hear from sufficiently many committee members.
% We conservatively set $\lambda_{step}$ to 20 seconds. 
% We set $\lambda_{stepvar}$, the estimated variance in BA* completion times, to 10 second.


